CyPhyHouse: A Programming, Simulation, and Deployment Toolchain for Heterogeneous Distributed Coordination

Programming languages, libraries, and development tools have transformed the application development processes for mobile computing and machine learning. This paper introduces the CyPhyHouse - a toolchain that aims to provide similar programming, debugging, and deployment benefits for distributed mobile robotic applications. Users can develop hardware-agnostic, distributed applications using the high-level, event driven Koord programming language, without requiring expertise in controller design or distributed network protocols. The modular, platform-independent middleware of CyPhyHouse implements these functionalities using standard algorithms for path planning (RRT), control (MPC), mutual exclusion, etc. A high-fidelity, scalable, multi-threaded simulator for Koord applications is developed to simulate the same application code for dozens of heterogeneous agents. The same compiled code can also be deployed on heterogeneous mobile platforms. The effectiveness of CyPhyHouse in improving the design cycles is explicitly illustrated in a robotic testbed through development, simulation, and deployment of a distributed task allocation application on in-house ground and aerial vehicles.

==> code/tasks_new.tex <==
using Motion:
  actuators:
    pos[] path
  sensors:
    pos psn
    boolean reached
local:
  boolean isOnTask
  Task myTask
  pos[] testRoute
  int i
    
allread:
  pos[] route
allwrite:
  Task[] list

Assign:
  pre: isOnTask == false
  eff: if allAssigned(list): stop
    else: atomic:
      for i = 0, length(list):
        if task.assigned$==$false:
          myTask$=$list[i]
            testRoute$=$findPath(Motion.psn,
                                 myTask.loc)
            if pathIsClear(route, testRoute, pid):
              isOnTask$=$true
              assign(myTask, pid)
              list[i]$=$myTask
              route[pid]$=$testRoute
              Motion.path$=$testRoute
            else:
              isOnTask$=$false
              route[pid]$=$[Motion.psn]
              
Complete:
    pre: isOnTask and Motion.reached
    eff: isOnTask$=$false
         route[pid]$=$[Motion.psn]
         
